Lumos3D: A Single-Forward Framework for Low-Light 3D Scene Restoration

Restoring 3D scenes with low-light conditions is challenging, and most existing methods depend on precomputed camera poses and scene-specific optimization, which greatly restricts their application to real-world scenarios. To overcome these limitations, we propose Lumos3D, a pose-free single-forward framework for 3D low-light scene restoration. First, we develop a cross-illumination distillation scheme, where a frozen teacher network takes normal-light ground truth images as input to distill accurate geometric information to the student model. Second, we define a Lumos loss to improve the restoration quality of the reconstructed 3D Gaussian space. Trained on a single dataset, Lumos3D performs inference in a purely feed-forward manner, directly restoring illumination and structure from unposed, low-light multi-view images without any per-scene training or optimization. Experiments on real-world datasets demonstrate that Lumos3D achieves competitive restoration results compared to scene-specific methods. Our codes are available at https://github.com/HanzhouLiu/Lumos3D.

==> section02_review.tex <==
\section{Background}

\subsection{3D Low-light Enhancement}
Neural Radiance Fields (NeRFs)~\cite{mildenhall2021nerf} have been adapted to low-light 3D scene restoration~\cite{wang2023lighting,qu2024lush,wang2024bilateral,cui2024aleth}. 
For example, Aleth-NeRF~\cite{cui2024aleth} introduces a concealing field that models illumination attenuation between objects and the viewer, enabling NeRF to reconstruct and render scenes under low-light and over-exposed conditions in a unified framework. 
Another line of research explores low-light enhancement within Gaussian Splatting (3DGS) frameworks~\cite{kerbl20233d}.
The recent Luminance-GS~\cite{cui2025luminance} extends 3DGS by adopting per-view color-matrix mapping and view-adaptive curve adjustment, achieving illumination-consistent novel view synthesis under low-light and over-exposed conditions.
However, these scene-specific methods typically rely on known camera poses and per-scene optimization, limiting their applications to real-world scenarios. 
In contrast, our proposed Lumos3D is trained on a single dataset and can be directly applied to unposed low-light scenes without any per-scene optimization.


\subsection{Single-Forward 3D Reconstruction}
Early neural-network models~\cite{ummenhofer2017demon,zhou2018deeptam,Teed2020DeepV2D:,wang2021multi} have demonstrated that end-to-end learning-based 3D reconstruction can be achieved.
Subsequently, large-scale models such as DUSt3R~\cite{wang2024dust3r} and MASt3R~\cite{leroy2024grounding} replace multi-stage SfM pipelines with single-pass predictions of geometry and poses.  
Later, Spann3R~\cite{wang2024spann3r}, CUT3R~\cite{wang2025continuous}, and MUSt3R~\cite{cabon2025must3r} further reduce reliance on classical optimization by incorporating memory or parallelized attention, albeit at relatively high computational cost. 
More recently, VGGT~\cite{wang2025vggt} introduces a novel Transformer architecture for joint multi-view inference of depth, pose, and point-maps.
AnySplat~\cite{jiang2025anysplat} extends VGGT into an efficient feed-forward 3DGS framework, bringing real-time novel-view synthesis within reach for unconstrained capture settings.
Inspired by these advancements, Lumos3D extends single-forward 3D reconstruction to low-light scenarios.

